Neural Fields in Visual Computing and Beyond

Recent advances in machine learning have created increasing interest in solving visual computing problems using a class of coordinate-based neural networks that parametrize physical properties of scenes or objects across space and time. These methods, which we call neural fields, have seen successful application in the synthesis of 3D shapes and image, animation of human bodies, 3D reconstruction, and pose estimation. However, due to rapid progress in a short time, many papers exist but a comprehensive review and formulation of the problem has not yet emerged. In this report, we address this limitation by providing context, mathematical grounding, and an extensive review of literature on neural fields. This report covers research along two dimensions. In Part I, we focus on techniques in neural fields by identifying common components of neural field methods, including different representations, architectures, forward mapping, and generalization methods. In Part II, we focus on applications of neural fields to different problems in visual computing, and beyond (e.g., robotics, audio). Our review shows the breadth of topics already covered in visual computing, both historically and in current incarnations, demonstrating the improved quality, flexibility, and capability brought by neural fields methods. Finally, we present a companion website that contributes a living version of this review that can be continually updated by the community.

==> figures/name.tex <==
\begin{figure*}[th!]
  \centering
  \includegraphics[width=0.95\linewidth]{images/part1.pdf}
  \label{fig:part1}
  \caption{Overview of a feed-forward neural field algorithm.}
\end{figure*}


==> figures/part2/digital_humans.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/digital_humans.pdf}
	\caption{\label{fig:digital_humans}Yang et al.~\cite{yang2021s3} jointly predict occupancy, skinning, and pose fields to animate reconstructed human avatars.}
	\vspace{-15pt}
\end{figure}


==> figures/part2/interactive_navigation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/part2/interactnav.pdf}
	\caption{}
	\vspace{-20pt}
	\label{fig:navigation}
\end{figure}


==> src/appendices/archived/common_loss_in_recon.tex <==
Common Loss Functions in 3D Reconstruction


%% YIHENG NOTE
% Geometry sparsity loss (useful for volume density)
% - To reconstruct hard surfaces, one can use the empty space loss and penalize volume density betwen the camera and object surface \cite{xian2020videonerf} $L=\int_{d_near}^{d_surface}{\sigma(x(t))} dt
% - Alternative
%% END YIHENG


==> src/appendices/archived/off_the_shelf.tex <==
Off-the-shelf methods used in neural fields:
- COLMAP
- SMPL
- MONOCULAR DEPTH ESTIMATION Networks
- RAFT
- 3DMM

==> tables/5.time_remap.tex <==
\begin{table}[t]
\centering
\begin{tabular}{l l}
\toprule
\textbf{Operation}           & \textbf{Functional Form}              \\
\midrule
Speed-up/Slow-down  & $f_\theta'(t) = f_\theta(a\cdot t)$ \\
Offset              & $f_\theta'(t) = f_\theta(t + b)$    \\
Reversal            & $f_\theta'(t) = f_\theta(-t)$       \\
\bottomrule
\end{tabular}
\caption{\label{tab:time_remap}Time remapping. $t$ is time, $a\in \mathbb{R}^+$ is a positive scalar, $b\in{R}$ is the offset.}
\vspace{-0.25cm}
\end{table}

==> tables/hybrid_rep.tex <==
\begin{table}[H]
\centering
\begin{tabular}{l l l}
\toprule
Characteristic      & Discrete Explicit & Neural Field \\
\midrule
Discrete/Continuous & Discrete             & Continuous      \\
Explicit/Implicit   & Explicit             & Implicit (most) \\
Memory Complexity   & High                 & Low             \\
Comp. Complexity    & Low                  & High            \\
\bottomrule
\end{tabular}
\caption{\label{tab:hybrid_rep}Characteristics of discrete explicit and neural field representations.\tt{I think we should be a bit careful about this table... for example computational complexity is not exactly low for a lot of data structures, and memory/complexity of a neural net is entirely architecture dependent, and data structures can be just as continuous as neural fields}}
\end{table}
